A Collaborative Ranking Model with Multiple Location-based Similarities for Venue Suggestion

Recommending venues plays a critical rule in satisfying users' needs on location-based social networks. Recent studies have explored the idea of adopting collaborative ranking (CR) for recommendation, combining the idea of learning to rank and collaborative filtering. However, CR suffers from the sparsity problem, mainly because it associates similar users based on exact matching of the venues in their check-in history. Even though research in collaborative filtering has shown that considering auxiliary information such as geographical influence, helps the model to alleviate the sparsity problem, the same direction still needs to be explored in CR. In this work, we present a CR framework that focuses on the top of the ranked list while integrating an arbitrary number of similarity functions between venues as it learns the model's parameters. We further introduce three example similarity measures based on venues' contents and locations. Incorporating cross-venue similarity measures into the model enhances the latent associations between users as similar venues are also taken into account while associating users with each other. Our experiments on the TREC Contextual Suggestion dataset show that our proposed CR model beats other state-of-the-art venue suggestion methods.

==> sec-analysis.tex <==
\section{Data Analysis}\label{sec-analysis}
% In this section, we introduce two real-world datasets of check-ins. Then, we conduct an extensive analysis of the datasets to explore the properties of check-in dynamics over time.
In this section, we conduct an extensive analysis of two real-world datasets to explore user preferences' dynamics over time.

\subsection{Data}
We use two real-world check-in datasets from Foursquare and Gowalla provided by~\citet{DBLP:conf/sigir/YuanCMSM13}. The Foursquare dataset originally consists of 342,850 check-ins of users in Singapore in the period of Aug. 2010 and Jul. 2011~\citep{DBLP:conf/sigir/YuanCMSM13}. The Gowalla dataset, on the other hand, includes 736,148 check-ins made by users in California and Nevada in the period of Feb. 2009 and Oct. 2010~\citep{DBLP:conf/sigir/YuanCMSM13}. Every check-in contains a user id, POI id, time, and geographical coordinates. For a fair comparison, we also use the preprocessed data as in~\citep{DBLP:conf/sigir/YuanCMSM13}. Users who have less than 5 check-ins, as well as POIs with less than 5 check-ins are removed from the datasets. Finally, we have 194,108 check-ins on Foursquare and 456,988 check-ins on Gowalla. We used the geographical coordinates of POIs to retrieve their corresponding categories such as bar, pizza place. More details are listed in Table~\ref{tab-stats}. Notice that multiple check-ins refer to the check-ins that were made by a particular user to a particular POI more than once. As shown in Table~\ref{tab-stats}, 45.51\% of check-ins on the Foursquare dataset refer to users visiting POIs more than once. In Gowalla, we observe fewer multiple check-ins, namely, 32.69\% of all check-ins. 

\begin{table}[t]
    \centering
    \caption{General statistics of the datasets}
    \begin{tabular}{l|l|l}
        \hline
         & \textbf{Foursquare} & \textbf{Gowalla} \\
        \hline
        \# of users & 2,231 & 10,162 \\\hline
        \# of POIs & 5,596 & 24,250 \\\hline
        \# of check-ins & 194,108 & 456,988 \\\hline
        Avg. POIs per user & 45.57 & 30.356 \\\hline
        Avg. users per POI & 18.90 & 12.69 \\\hline
        Multiple check-ins & 45.51\% & 32.69\% \\ \hline
        Density & 0.0081 & 0.0012 \\
        \hline
    \end{tabular}
    \label{tab-stats}
\end{table}

% \subsection{Empirical Analysis}

% \textbf{Long-tailed properties and data sparsity.}
% The distribution of users' check-ins on Gowalla is shown in \autoref{fig-power}. We also show the cumulative distribution functions for users on Gowalla \autoref{fig-power}. Note that since POIs exhibit a similar distribution we only plot users. Also, the distributions on both datasets are similar. As we can see, the distributions follow power-laws. In fact, these figures show that only a fraction of users accounts for the majority of the datasets. Existence of ``power users"~\citep{DBLP:journals/corr/abs-1304-4523} is usually observed in such datasets which again explains why POI recommendation datasets are sparse and have a very low density as in \autoref{tab-stats}. The figure of the right indicates that while there are a few users with numerous check-ins, the majority of users do not check-in as much. Therefore, considering POIs that a user has checked in as positive training examples, and POIs that a user has not checked in as negative training examples can significantly help a system to alleviate data sparsity. One can argue that considering all POIs as training examples for users my affect the model's efficiency. While this argument is valid, designing an efficient optimization algorithm is out of the scope of this article. However, one possible strategy could be selective negative sampling (e.g., considering unvisited POIs in the geographical vicinity as negative examples). 
% % Interestingly, the last two rows of \autoref{fig-power} supports our argument. As we can see, only a fraction of POIs account for the majority of check-ins. This suggests that a model that only considers visited POIs as training examples could potentially be biased toward recommending \textit{power POIs}. Therefore, our proposed model considers both visited and unvisited POIs for training.


% % \begin{figure} \centering
% % \begin{tabular}{cc}
% % \textbf{Foursquare} & \textbf{Gowalla} \\
% % \includegraphics[height=0.35\columnwidth]{figures/foursquare_user_count_count} & \includegraphics[height=0.35\columnwidth]{figures/gowalla_user_count_count}\\
% % \includegraphics[height=0.35\columnwidth]{figures/foursquare_user_cum_dist} & \includegraphics[height=0.35\columnwidth]{figures/gowalla_user_cum_dist}\\
% % \includegraphics[height=0.35\columnwidth]{figures/foursquare_venue_count_count} & \includegraphics[height=0.35\columnwidth]{figures/gowalla_venue_count_count}\\
% % \includegraphics[height=0.35\columnwidth]{figures/foursquare_venue_cum_dist} & \includegraphics[height=0.35\columnwidth]{figures/gowalla_venue_cum_dist} \\
% % \end{tabular}
% % \caption{The distribution of item check-ins with respect to users (first two rows) and POIs (last two rows). The distributions for both datasets follow a power-law distribution (Foursquare on the left, Gowalla on the right). The cumulative distribution function plots on the second and fourth rows demonstrate the proportion of users and POIs that account for the total number of check-ins, respectively. Existence of power users and power POIs is evident for both datasets.} 
% % \label{fig-power}
% % \end{figure}

% \begin{figure} \centering
% \begin{tabular}{cc}
% \includegraphics[height=0.40\textwidth]{figures/gowalla_user_count_count} & \includegraphics[height=0.40\textwidth]{figures/gowalla_user_cum_dist}
% \end{tabular}
% \caption{The distribution of check-ins with respect to users (on the left) and the cumulative distribution function plot (on the right) which demonstrates the proportion of users that account for the total number of check-ins, respectively.} 
% \label{fig-power}
% \end{figure}

% \textbf{Users activities and interests are time-dependent.}\label{sec-time-analysis}

\subsection{Time-Dependency of User Activities and Interests}\label{sec-time-analysis}

Many studies analyzed users activity patterns over time~\citep{DBLP:conf/cikm/YuanCS14,DBLP:conf/sigir/YuanCMSM13,DBLP:conf/icdm/YaoFLLX16,DBLP:conf/recsys/GaoTHL13,DBLP:conf/cikm/DeveaudAMO15}. However, user activities have been mostly studied at an hourly basis. We conduct a long-term user activity analysis, namely we study the user behavior over several months. The monthly analysis allows us to realize the long-term shift of users interest. Users' interests could evolve over time while sustaining their personal patterns. For instance, a teenager who reaches the legal age of drinking starts going to bars (long-term interest shift), whereas an adult user often chooses to travel on every Easter (personal pattern). \autoref{fig-hist} depicts the distribution of check-ins of both datasets every month. There is a significant shift of activity on each month. For instance, we observe that the number of check-ins increases from Feb. to Jul. in both datasets. 
Next, we report further analysis only on Gowalla, as we observed similar properties when analyzing the Foursquare dataset. 
\autoref{fig-popularity} shows the popularity of the top-8 venue categories. As we can see, before Oct. 2009 we observe dramatic shifts of popularity. However, after Oct. 2009, the top categories exhibit a rather more stable popularity pattern as the dataset grows. Interestingly, we still can observe popularity shifts between ``Coffee Shop", ``American", ``Mexican", ``City Park", and ``Asian". This suggests that users exhibit a time-dependent pattern in visiting even the most popular categories of POIs. 

\autoref{fig-vars} shows the activity of two samples of users in a long period. It also shows how the popularity of two samples of POI categories change over time. Note that, all the plots of \autoref{fig-vars} illustrate the distribution of each user or category over time, that is, for each user or category, summing all the values of Y over time (X) equals to 1. We compute the variance of check-ins for both users and categories. Then, we pick the ones with the lowest in \autoref{fig-vars}a \& c and the ones with the highest variances in \autoref{fig-vars}b \& d. Our aim is to pick some representative user and categories from either end of the spectrum. As we can see, even users who are supposed to be the most stable users (\autoref{fig-vars}a) exhibit very time-dependent check-in patterns. It is worth noting that we ignored users with less than 50 check-ins for plotting \autoref{fig-vars}b, as those users mostly appear once in the dataset and hence are listed among the top variant users. However, we still observe that the users with high check-in variance are those who appear a few times and have less regular check-in behavior. This suggests that the more active a user is, the less variant her check-in pattern is. We also observed a negative correlation between the users' check-in variance and quantity (Spearman: $-$0.5583) which supports our assumption. As for the POI categories, \autoref{fig-vars}c depicts the least variant categories. First, all of the categories relate to users' daily activities, for example going to a coffee shop or sandwich store. These categories are more time-independent since they are less affected by season change or weather conditions. Likewise what we observed for users, more popular categories are also less time-variant. In fact, we found a negative correlation between POI categories variance and popularity (Spearman: $-$0.8411). On the other hand, the most time-variant categories (\autoref{fig-vars}d) are less popular and mostly dependent on weather, such as Ski Shop,  and political events, like for example Democratic Event. 

All our observations suggest that there is an underlying temporal pattern in check-in activities from the perspective of both users and place categories. As we argued, check-in variance reveals meaningful information and thus we design our model focusing on these aspects.

\begin{figure}[t] \centering
\begin{tabular}{cc}
\textbf{Foursquare} & \textbf{Gowalla} \\
\includegraphics[width=0.49\textwidth]{figures/foursquare_hist} & \includegraphics[width=0.49\textwidth]{figures/gowalla_hist}\\
\end{tabular}
\caption{Number of check-ins per month on Foursquare and Gowalla.} 
\label{fig-hist}
\end{figure}

\begin{figure}[t] \centering
\includegraphics[width=0.8\textwidth]{figures/gowalla_category_popularity}
\caption{Popularity of the top-8 categories over time on Gowalla.} 
\label{fig-popularity}
\end{figure}

\begin{figure}[t] \centering
\begin{tabular}{cc}
\includegraphics[width=0.49\textwidth]{figures/gowalla_least_variant_users} & \includegraphics[width=0.49\textwidth]{figures/gowalla_most_variant_users}\\
(a) & (b) \\
\includegraphics[width=0.49\textwidth]{figures/gowalla_least_variant} & \includegraphics[width=0.49\textwidth]{figures/gowalla_most_variant} \\
(c) & (d) \\
\end{tabular}
\caption{Check-in distribution of users and POI categories over time. Figures (a) and (c) depict the least time-variant users and POI categories, respectively. Figures (b) and (d), in contrast, show the distribution of the most time-variant users and POI categories, respectively.} 
\label{fig-vars}
\end{figure}

% \textbf{Users tend to visit the same venues multiple times.}

\subsection{Users' Multiple Check-ins}

As we discussed earlier in Section~\ref{sec-introduction}, a good indicator of a user's preference is the fact that she visits the same POI multiple times. 
% \begin{definition} 
% \label{def-multi}
Multiple check-in between a users $\rho$ and a venue $l$ occurs if $\rho$ visits $l$ more than once.
% \end{definition}
Other studies assumed multiple check-ins as an implicit feedback and demonstrated its effectiveness~\citep{DBLP:conf/sigir/LiCLPK15}. We also observed that a considerable amount of check-ins are multiple check-ins (\autoref{tab-stats}). We randomly picked 50 users from the top-500 users of Gowalla. \autoref{fig-multi} shows the quantity of single check-ins as well as multiple check-ins of the sample users. As we can see, users spend a considerable amount of their time visiting POIs they have visited before. In fact, multiple check-ins constitute 20\% of check-ins of an average user on Gowalla (with a standard deviation of 21). According to \autoref{fig-multi}, the more active a user is, the more multiple check-ins she has. We calculated the correlation between the number of check-ins and the percentage of multiple check-ins per user. Interestingly, we observe that there is a positive correlation (Spearman: +0.4257) between the two variables, supporting our assumption. Based on these observations, we confirm that multiple check-ins provide valuable information regarding users' preference and since they account for a considerable amount of the datasets, we design our model with a focus on them.

\begin{figure} \centering
\includegraphics[width=0.8\textwidth]{figures/gowalla_multi_single_checkin}
\caption{Check-in histogram of 50 randomly-sampled users from the top-500 users of Gowalla. For each user, the red bar denotes the number of multiple check-ins, while the blue bar denotes the number of single check-ins.} 
\label{fig-multi}
\end{figure}





